OmniAlpha: Aligning Transparency-Aware Generation via Multi-Task Unified Reinforcement Learning

Transparency-aware generation requires modeling not only RGB appearance but also alpha-based opacity and cross-layer composition, which are essential for tasks such as image matting, object removal, layer decomposition, and multi-layer content creation. However, existing RGBA-related methods remain largely fragmented, with separate pipelines designed for individual tasks. While a unified model is desirable, supervised fine-tuning alone is insufficient, as localized regression objectives cannot directly optimize the compositional fidelity, alpha-boundary precision, and structural consistency required for high-quality RGBA generation. To address this, we propose OmniAlpha, a unified multi-task reinforcement learning framework for transparency-aware generation and manipulation. OmniAlpha combines an end-to-end alpha-aware VAE and a sequence-to-sequence Diffusion Transformer, with a bi-directional layer axis in positional encoding to jointly model multiple RGBA inputs and outputs within a single forward pass. Built on a multi-task SFT cold start, it further performs GRPO-style post-training with layer-aware rewards defined on decoded RGBA outputs, enabling direct optimization of cross-layer coherence and fine transparency details. Experiments across five categories of transparency-aware tasks show that OmniAlpha consistently outperforms its unified SFT baseline and achieves strong performance against specialized expert models, including a 9.07% relative reduction in RGB L1 on layer decomposition and 74%/68% improvements over conventional matting tools on SAD/Grad for automatic matting.

==> app/code.tex <==
\clearpage
\section{Core Pipeline Codes}

\begin{tcolorbox}[
    colback=gray!5,        % 背景浅灰
    colframe=gray!60,      % 边框浅灰（不会太黑）
    boxrule=0.5pt,         % 边框宽度更细
    arc=5pt,               % 圆角更柔和
    left=4pt,right=4pt,top=4pt,bottom=4pt,
    breakable
]
\begin{Verbatim}[fontsize=\tiny,breaklines=true,breakanywhere=true,breaksymbol={}]
from dataclasses import dataclass

from torch import nn
from PIL import Image

# from diffusers.pipelines.qwenimage.pipeline_qwenimage_edit import *
from diffusers.pipelines.qwenimage.pipeline_qwenimage_edit_plus import *
# from diffusers import QwenImageEditPlusPipeline

@dataclass
class QwenImageEditModules:
    scheduler: FlowMatchEulerDiscreteScheduler
    vae: AutoencoderKLQwenImage
    text_encoder: Qwen2_5_VLForConditionalGeneration
    tokenizer: Qwen2Tokenizer
    processor: Qwen2VLProcessor
    transformer: QwenImageTransformer2DModel
    
    @classmethod
    def from_pipeline(cls, pipeline: QwenImageEditPlusPipeline):
        return cls(
            scheduler=pipeline.scheduler,
            vae=pipeline.vae,
            text_encoder=pipeline.text_encoder,
            tokenizer=pipeline.tokenizer,
            processor=pipeline.processor,
            transformer=pipeline.transformer,
        )
        
    def requires_grad_(self, requires_grad: bool):
        self.transformer.requires_grad_(requires_grad)
        self.text_encoder.requires_grad_(requires_grad)
        self.vae.requires_grad_(requires_grad)
    
    def to_dict(self):
        return {**self.__dict__}
    
    def to(self, *args, **kwargs):
        for module in self.to_dict().values():
            if isinstance(module, nn.Module):
                module.to(*args, **kwargs)




class CustomQwenImageEditPlusPipeline(QwenImageEditPlusPipeline):


    @staticmethod
    # Modified from diffusers.pipelines.qwenimage.pipeline_qwenimage.QwenImagePipeline._pack_latents
    def pack_latents_multi_frames(latents):
        """
        B, C, F, H, W -> B, F * H/2 * W/2, 4C
        """
        B, C, F, H, W = latents.shape
        latents = latents.view(B, C, F, H // 2, 2, W // 2, 2)
        latents = latents.permute(0, 2, 3, 5, 1, 4, 6) # B, F, H/2, W/2, C, 2, 2
        latents = latents.reshape(B, F * (H // 2) * (W // 2), C * 4) # B, F * H/2 * W/2, 4C
        return latents

    @staticmethod
    # Modified from diffusers.pipelines.qwenimage.pipeline_qwenimage.QwenImagePipeline._unpack_latents
    def unpack_latents_multi_frames(latents, frames, height_latents, width_latents):
        """
        B, F * H/2 * W/2, 4C -> B, C, F, H, W
        """
        B, L, C4 = latents.shape
        F = frames
        H = height_latents
        W = width_latents
        latents = latents.view(B, F, H // 2, W // 2, C4 // 4, 2, 2)
        latents = latents.permute(0, 4, 1, 2, 5, 3, 6) # B, C, F, H/2, 2, W/2, 2
        latents = latents.reshape(B, C4 // 4, F, H, W)
        return latents

    def _get_qwen_prompt_embeds(
        self,
        prompt: Union[str, List[str]] = None,
        image: Optional[torch.Tensor] = None,
        device: Optional[torch.device] = None,
        dtype: Optional[torch.dtype] = None,
    ):
        device = device or self._execution_device
        dtype = dtype or self.text_encoder.dtype

        prompt = [prompt] if isinstance(prompt, str) else prompt
        img_prompt_template = "Picture {}: <|vision_start|><|image_pad|><|vision_end|>"
        if isinstance(image, list):
            base_img_prompt = ""
            for i, img in enumerate(image):
                base_img_prompt += img_prompt_template.format(i + 1)
        elif image is not None:
            base_img_prompt = img_prompt_template.format(1)
        else:
            base_img_prompt = ""

        template = self.prompt_template_encode

        drop_idx = self.prompt_template_encode_start_idx
        txt = [template.format(base_img_prompt + e) for e in prompt]

        model_inputs = self.processor(
            text=txt,
            images=image,
            padding=True,
            return_tensors="pt",
        ).to(device)

        outputs = self.text_encoder(
            input_ids=model_inputs.input_ids,
            attention_mask=model_inputs.attention_mask,
            pixel_values=model_inputs.pixel_values if image else None,
            image_grid_thw=model_inputs.image_grid_thw if image else None,
            output_hidden_states=True,
        )

        hidden_states = outputs.hidden_states[-1]
        split_hidden_states = self._extract_masked_hidden(hidden_states, model_inputs.attention_mask)
        split_hidden_states = [e[drop_idx:] for e in split_hidden_states]
        attn_mask_list = [torch.ones(e.size(0), dtype=torch.long, device=e.device) for e in split_hidden_states]
        max_seq_len = max([e.size(0) for e in split_hidden_states])
        prompt_embeds = torch.stack(
            [torch.cat([u, u.new_zeros(max_seq_len - u.size(0), u.size(1))]) for u in split_hidden_states]
        )
        encoder_attention_mask = torch.stack(
            [torch.cat([u, u.new_zeros(max_seq_len - u.size(0))]) for u in attn_mask_list]
        )

        prompt_embeds = prompt_embeds.to(dtype=dtype, device=device)

        return prompt_embeds, encoder_attention_mask
    
    def prepare_condition_image(self, img: Image.Image, reshape: bool = True):
        if img.mode != "RGB":
            img = img.convert("RGBA")
            bg = Image.new("RGB", img.size, (255, 255, 255))
            bg.paste(img, (0, 0), img)
            img = bg
        image_width, image_height = img.size
        new_width, new_height = calculate_dimensions(
            CONDITION_IMAGE_SIZE if reshape else image_width * image_height, 
            image_width / image_height
        )
        return (
            self.image_processor.resize(img, new_width, new_height),
            (new_width, new_height)
        )
    
    def prepare_vae_image(self, img: Image.Image, reshape: bool = True):
        # RETURN: B=1 C F=1 H W
        image_width, image_height = img.size
        new_width, new_height = calculate_dimensions(
            VAE_IMAGE_SIZE if reshape else image_width * image_height, 
            image_width / image_height
        )
        return (
            self.image_processor.preprocess(img, new_width, new_height).unsqueeze(2),
            (new_width, new_height)
        )
        
    def prepare_images(
        self,
        images: Union[None, Image.Image, List[Image.Image]], 
        prepare_type: str,
        reshape: bool = True
    ):
        assert prepare_type in ['condition', 'vae'], "prepare_type must be either 'condition' or 'vae'"
        if images is None:
            return [], []
        
        shapes = []
        prepared_images = []
        
        if not isinstance(images, list):
            images = [images]
            
        for img in images:
            img, shape = {
                'condition': self.prepare_condition_image,
                'vae': self.prepare_vae_image
            }[prepare_type](img, reshape)
            prepared_images.append(img)
            shapes.append(shape)
        
        return prepared_images, shapes

    def prepare_latents(
        self,
        images,
        batch_size,
        num_channels_latents,
        height,
        width,
        dtype,
        device,
        generator,
        latents=None,
        frames=1,
    ):
        # VAE applies 8x compression on images but we must also account for packing which requires
        # latent height and width to be divisible by 2.
        height = 2 * (int(height) // (self.vae_scale_factor * 2))
        width = 2 * (int(width) // (self.vae_scale_factor * 2))

        image_latents = None
        if images is not None:
            if not isinstance(images, list):
                images = [images]
            all_image_latents = []
            for image in images:
                image = image.to(device=device, dtype=dtype)
                if image.shape[1] != self.latent_channels:
                    image_latents = self._encode_vae_image(image=image, generator=generator)
                else:
                    image_latents = image
                if batch_size > image_latents.shape[0] and batch_size % image_latents.shape[0] == 0:
                    # expand init_latents for batch_size
                    additional_image_per_prompt = batch_size // image_latents.shape[0]
                    image_latents = torch.cat([image_latents] * additional_image_per_prompt, dim=0)
                elif batch_size > image_latents.shape[0] and batch_size % image_latents.shape[0] != 0:
                    raise ValueError(
                        f"Cannot duplicate `image` of batch size {image_latents.shape[0]} to {batch_size} text prompts."
                    )
                else:
                    image_latents = torch.cat([image_latents], dim=0)

                image_latent_height, image_latent_width = image_latents.shape[3:]
                image_latents = self._pack_latents(
                    image_latents, batch_size, num_channels_latents, image_latent_height, image_latent_width
                )
                all_image_latents.append(image_latents)
            image_latents = torch.cat(all_image_latents, dim=1)

        if isinstance(generator, list) and len(generator) != batch_size:
            raise ValueError(
                f"You have passed a list of generators of length {len(generator)}, but requested an effective batch"
                f" size of {batch_size}. Make sure the batch size matches the length of the generators."
            )
        if latents is None:
            shape = (batch_size, num_channels_latents, frames, height, width)
            latents = randn_tensor(shape, generator=generator, device=device, dtype=dtype)
            latents = self.pack_latents_multi_frames(latents)
        else:
            latents = latents.to(device=device, dtype=dtype)

        return latents, image_latents
    
    @torch.no_grad()
    @replace_example_docstring(EXAMPLE_DOC_STRING)
    def __call__(
        self,
        image: Optional[PipelineImageInput] = None,
        prompt: Union[str, List[str]] = None,
        negative_prompt: Union[str, List[str]] = None,
        true_cfg_scale: float = 4.0,
        height: Optional[int] = None,
        width: Optional[int] = None,
        num_inference_steps: int = 50,
        sigmas: Optional[List[float]] = None,
        guidance_scale: Optional[float] = None,
        num_images_per_prompt: int = 1,
        generator: Optional[Union[torch.Generator, List[torch.Generator]]] = None,
        latents: Optional[torch.Tensor] = None,
        prompt_embeds: Optional[torch.Tensor] = None,
        prompt_embeds_mask: Optional[torch.Tensor] = None,
        negative_prompt_embeds: Optional[torch.Tensor] = None,
        negative_prompt_embeds_mask: Optional[torch.Tensor] = None,
        output_type: Optional[str] = "pil",
        return_dict: bool = True,
        attention_kwargs: Optional[Dict[str, Any]] = None,
        callback_on_step_end: Optional[Callable[[int, int, Dict], None]] = None,
        callback_on_step_end_tensor_inputs: List[str] = ["latents"],
        max_sequence_length: int = 512,
        debug: bool = False,
        frames: int = 1,
        reshape: bool = False,
    ):
        if image is not None:
            one_image = image[0] if isinstance(image, list) else image
            # image_size = one_image.shape if isinstance(one_image, torch.Tensor) else one_image.size
            if isinstance(one_image, torch.Tensor):
                raise NotImplementedError("Pass PIL.Image.Image instead")
                # TODO: support tensor in the future versions
                input_width = one_image.shape[-1]
                input_height = one_image.shape[-2]
            else:
                input_width = one_image.size[0]
                input_height = one_image.size[1]
            calculated_width, calculated_height = calculate_dimensions(1024 * 1024, input_width / input_height)
            height = height or calculated_height
            width = width or calculated_width
        else:
            height = height or self.default_sample_size * self.vae_scale_factor
            width = width or self.default_sample_size * self.vae_scale_factor

        multiple_of = self.vae_scale_factor * 2
        width = width // multiple_of * multiple_of
        height = height // multiple_of * multiple_of

        # 1. Check inputs. Raise error if not correct
        self.check_inputs(
            prompt,
            height,
            width,
            negative_prompt=negative_prompt,
            prompt_embeds=prompt_embeds,
            negative_prompt_embeds=negative_prompt_embeds,
            prompt_embeds_mask=prompt_embeds_mask,
            negative_prompt_embeds_mask=negative_prompt_embeds_mask,
            callback_on_step_end_tensor_inputs=callback_on_step_end_tensor_inputs,
            max_sequence_length=max_sequence_length,
        )

        self._guidance_scale = guidance_scale
        self._attention_kwargs = attention_kwargs
        self._current_timestep = None
        self._interrupt = False

        # 2. Define call parameters
        if prompt is not None and isinstance(prompt, str):
            batch_size = 1
        elif prompt is not None and isinstance(prompt, list):
            batch_size = len(prompt)
        else:
            batch_size = prompt_embeds.shape[0]

        device = self._execution_device
        # 3. Preprocess 
        
        if debug:
            print("DEBUG 3")
            
        if (isinstance(image, torch.Tensor) and image.size(1) == self.latent_channels):
            raise NotImplementedError
        
        has_condition = image is not None
            
        condition_images, condition_image_sizes = self.prepare_images(
            images=image,
            prepare_type='condition',
            reshape=reshape
        )
        
        vae_images, vae_image_sizes = self.prepare_images(
            images=image,
            prepare_type='vae',
            reshape=reshape
        )
        
        if debug:
            print(f"{vae_images[0].shape=}, {vae_image_sizes=}")
        
        has_neg_prompt = negative_prompt is not None or (
            negative_prompt_embeds is not None and negative_prompt_embeds_mask is not None
        )

        if true_cfg_scale > 1 and not has_neg_prompt:
            logger.warning(
                f"true_cfg_scale is passed as {true_cfg_scale}, but classifier-free guidance is not enabled since no negative_prompt is provided."
            )
        elif true_cfg_scale <= 1 and has_neg_prompt:
            logger.warning(
                " negative_prompt is passed but classifier-free guidance is not enabled since true_cfg_scale <= 1"
            )

        do_true_cfg = true_cfg_scale > 1 and has_neg_prompt
        if debug:
            print(f"{prompt=}")
        prompt_embeds, prompt_embeds_mask = self.encode_prompt(
            image=condition_images if has_condition else None,
            prompt=prompt,
            prompt_embeds=prompt_embeds,
            prompt_embeds_mask=prompt_embeds_mask,
            device=device,
            num_images_per_prompt=num_images_per_prompt,
            max_sequence_length=max_sequence_length,
        )
        
        if debug:
            print(f"{condition_images=}")
            print(f"{prompt_embeds.shape=}, {prompt_embeds_mask.shape=}")
            print(f"{prompt_embeds.min()=}, {prompt_embeds.max()=}")
            print(f"{prompt_embeds.std()=}, {prompt_embeds.mean()=}")
        
        if do_true_cfg:
            negative_prompt_embeds, negative_prompt_embeds_mask = self.encode_prompt(
                image=condition_images if has_condition else None,
                prompt=negative_prompt,
                prompt_embeds=negative_prompt_embeds,
                prompt_embeds_mask=negative_prompt_embeds_mask,
                device=device,
                num_images_per_prompt=num_images_per_prompt,
                max_sequence_length=max_sequence_length,
            )

        # 4. Prepare latent variables
        num_channels_latents = self.transformer.config.in_channels // 4
        latents, image_latents = self.prepare_latents(
            vae_images if has_condition else None,
            batch_size * num_images_per_prompt,
            num_channels_latents,
            height,
            width,
            prompt_embeds.dtype,
            device,
            generator,
            latents,
            frames,
        )
        latent_height = height // self.vae_scale_factor
        latent_width = width // self.vae_scale_factor
        assert latents.shape[1] == frames * latent_height // 2 * latent_width // 2, "Latents shape is incorrect."
        img_shapes = [
            [
                *([(1, latent_height // 2, latent_width // 2)] * frames),
                *[
                    (1, vae_height // self.vae_scale_factor // 2, vae_width // self.vae_scale_factor // 2)
                    for vae_width, vae_height in vae_image_sizes
                ],
            ]
        ] * batch_size

        # 5. Prepare timesteps
        sigmas = np.linspace(1.0, 1 / num_inference_steps, num_inference_steps) if sigmas is None else sigmas
        image_seq_len = latents.shape[1]
        mu = calculate_shift(
            image_seq_len,
            self.scheduler.config.get("base_image_seq_len", 256),
            self.scheduler.config.get("max_image_seq_len", 4096),
            self.scheduler.config.get("base_shift", 0.5),
            self.scheduler.config.get("max_shift", 1.15),
        )
        timesteps, num_inference_steps = retrieve_timesteps(
            self.scheduler,
            num_inference_steps,
            device,
            sigmas=sigmas,
            mu=mu,
        )
        num_warmup_steps = max(len(timesteps) - num_inference_steps * self.scheduler.order, 0)
        self._num_timesteps = len(timesteps)

        # handle guidance
        if self.transformer.config.guidance_embeds and guidance_scale is None:
            raise ValueError("guidance_scale is required for guidance-distilled model.")
        elif self.transformer.config.guidance_embeds:
            guidance = torch.full([1], guidance_scale, device=device, dtype=torch.float32)
            guidance = guidance.expand(latents.shape[0])
        elif not self.transformer.config.guidance_embeds and guidance_scale is not None:
            logger.warning(
                f"guidance_scale is passed as {guidance_scale}, but ignored since the model is not guidance-distilled."
            )
            guidance = None
        elif not self.transformer.config.guidance_embeds and guidance_scale is None:
            guidance = None

        if self.attention_kwargs is None:
            self._attention_kwargs = {}

        txt_seq_lens = prompt_embeds_mask.sum(dim=1).tolist() if prompt_embeds_mask is not None else None
        negative_txt_seq_lens = (
            negative_prompt_embeds_mask.sum(dim=1).tolist() if negative_prompt_embeds_mask is not None else None
        )

        # 6. Denoising loop
        self.scheduler.set_begin_index(0)
        with self.progress_bar(total=num_inference_steps) as progress_bar:
            for i, t in enumerate(timesteps):
                if self.interrupt:
                    continue

                self._current_timestep = t

                latent_model_input = latents
                if image_latents is not None:
                    latent_model_input = torch.cat([latents, image_latents], dim=1)

                # broadcast to batch dimension in a way that's compatible with ONNX/Core ML
                timestep = t.expand(latents.shape[0]).to(latents.dtype)
                with self.transformer.cache_context("cond"):
                    noise_pred = self.transformer(
                        hidden_states=latent_model_input,
                        timestep=timestep / 1000,
                        guidance=guidance,
                        encoder_hidden_states_mask=prompt_embeds_mask,
                        encoder_hidden_states=prompt_embeds,
                        img_shapes=img_shapes,
                        txt_seq_lens=txt_seq_lens,
                        attention_kwargs=self.attention_kwargs,
                        return_dict=False,
                    )[0]
                    noise_pred = noise_pred[:, : latents.size(1)]

                if do_true_cfg:
                    with self.transformer.cache_context("uncond"):
                        neg_noise_pred = self.transformer(
                            hidden_states=latent_model_input,
                            timestep=timestep / 1000,
                            guidance=guidance,
                            encoder_hidden_states_mask=negative_prompt_embeds_mask,
                            encoder_hidden_states=negative_prompt_embeds,
                            img_shapes=img_shapes,
                            txt_seq_lens=negative_txt_seq_lens,
                            attention_kwargs=self.attention_kwargs,
                            return_dict=False,
                        )[0]
                    neg_noise_pred = neg_noise_pred[:, : latents.size(1)]
                    # neg_noise_pred = neg_noise_pred[:, -latents.size(1):]
                    comb_pred = neg_noise_pred + true_cfg_scale * (noise_pred - neg_noise_pred)

                    cond_norm = torch.norm(noise_pred, dim=-1, keepdim=True)
                    noise_norm = torch.norm(comb_pred, dim=-1, keepdim=True)
                    noise_pred = comb_pred * (cond_norm / noise_norm)

                # compute the previous noisy sample x_t -> x_t-1
                latents_dtype = latents.dtype
                latents = self.scheduler.step(noise_pred, t, latents, return_dict=False)[0]

                if latents.dtype != latents_dtype:
                    if torch.backends.mps.is_available():
                        latents = latents.to(latents_dtype)

                if callback_on_step_end is not None:
                    callback_kwargs = {}
                    for k in callback_on_step_end_tensor_inputs:
                        callback_kwargs[k] = locals()[k]
                    callback_outputs = callback_on_step_end(self, i, t, callback_kwargs)

                    latents = callback_outputs.pop("latents", latents)
                    prompt_embeds = callback_outputs.pop("prompt_embeds", prompt_embeds)

                # call the callback, if provided
                if i == len(timesteps) - 1 or ((i + 1) > num_warmup_steps and (i + 1) % self.scheduler.order == 0):
                    progress_bar.update()

                if XLA_AVAILABLE:
                    xm.mark_step()

        self._current_timestep = None
        if output_type == "latent":
            image = latents
        else:
            if debug:
                print(f"{latents.shape=}, {frames=}, {latent_height=}, {latent_width=}")
            latents = self.unpack_latents_multi_frames(latents, frames, latent_height, latent_width) # B, C, F, H, W
            latents = latents.permute(0, 2, 1, 3, 4) # B, F, C, H, W
            B, F, C, H, W = latents.shape
            latents = latents.view(B * F, C, 1, H, W)
            latents = latents.to(self.vae.dtype)
            latents_mean = (
                torch.tensor(self.vae.config.latents_mean)
                .view(1, self.vae.config.z_dim, 1, 1, 1)
                .to(latents.device, latents.dtype)
            )
            latents_std = 1.0 / torch.tensor(self.vae.config.latents_std).view(1, self.vae.config.z_dim, 1, 1, 1).to(
                latents.device, latents.dtype
            )
            latents = latents / latents_std + latents_mean
            image = self.vae.decode(latents, return_dict=False)[0][:, :, 0]
            image = self.image_processor.postprocess(image, output_type=output_type)
                

        # Offload all models
        self.maybe_free_model_hooks()

        if not return_dict:
            return (image,)

        return QwenImagePipelineOutput(images=image)
\end{Verbatim}
\end{tcolorbox}
